Graph InfoClust: Leveraging cluster-level node information for unsupervised graph representation learning

Unsupervised (or self-supervised) graph representation learning is essential to facilitate various graph data mining tasks when external supervision is unavailable. The challenge is to encode the information about the graph structure and the attributes associated with the nodes and edges into a low dimensional space. Most existing unsupervised methods promote similar representations across nodes that are topologically close. Recently, it was shown that leveraging additional graph-level information, e.g., information that is shared among all nodes, encourages the representations to be mindful of the global properties of the graph, which greatly improves their quality. However, in most graphs, there is significantly more structure that can be captured, e.g., nodes tend to belong to (multiple) clusters that represent structurally similar nodes. Motivated by this observation, we propose a graph representation learning method called Graph InfoClust (GIC), that seeks to additionally capture cluster-level information content. These clusters are computed by a differentiable K-means method and are jointly optimized by maximizing the mutual information between nodes of the same clusters. This optimization leads the node representations to capture richer information and nodal interactions, which improves their quality. Experiments show that GIC outperforms state-of-art methods in various downstream tasks (node classification, link prediction, and node clustering) with a 0.9% to 6.1% gain over the best competing approach, on average.

==> figs/clusts.tex <==
\begin{tikzpicture}[every node/.style={scale=2}]
\begin{axis}[legend style={at={(.9,0.9),anchor=north east}},
             legend style={legend pos=outer north east,}, xtick={1,3,5,7,9}, xticklabels={0.5,2,7,15,30}, title={CORA},ylabel={Acc (\%)}, xlabel={$K/$\#nodes (\%)}, ytick={81,82,83,84,85}, ymin=81, ymax=85,
]

\addplot[mark=diamond*,violet] coordinates {
    (1,82.8)
    (2,83.2)
    (3,83.5)
    (4,82.6)
    (5,82.4)
    (6, 83.0)
    (7, 83.4)
    (8,83.4)
    (9,82.2)
    
};
\addplot[mark=diamond*,blue] coordinates {
    (1,82.4)
    (2,83.0)
    (3,82.8)
    (4,82.5)
    (5,83.3)
    (6, 83.8)
    (7, 83.3)
    (8,82.7)
    (9,83.0)
    
};
\addplot[mark=diamond*,cyan] coordinates {
    (1,83.5)
    (2,84.0)
    (3,83.1)
    (4,83.4)
    (5,83.2)
    (6, 83.9)
    (7, 83.2)
    (8,83.5)
    (9,82.9)
    
};

%\addlegendentry{$\beta=1$}
\addplot[mark=diamond*,green] coordinates {
    (1,83.2)
    (2,83.8)
    (3,83.5)
    (4,84.3)
    (5, 83.3)
    (6, 83.8)
    (7,83.7)
    (8,83.1)
    (9,83.3)
};
\addplot[mark=diamond*,red] coordinates {
    (1,83.5)
    (2,84.0)
    (3,83.3)
    (4,83.3)
    (5, 83.4)
    (6, 84.0)
    (7,83.3)
    (8,83.4)
    (9,83.2)
};
%\addlegendentry{$\beta=100$}


\end{axis}
\end{tikzpicture}

\begin{tikzpicture}[every node/.style={scale=2}]
\begin{axis}[legend style={at={(.9,0.9),anchor=north east}},
             legend style={cells={anchor=east}, legend pos=outer north east,}, xtick={2,4,6,8}, xticklabels={1,5,10,20}, title={CiteSeer}, xlabel={$K/$\#nodes (\%)}, ytick={65.5,66.5,67.5,68.5,69.5}, ymin=65.5, ymax=69.5,
]
\addplot[mark=diamond*,thick,violet] coordinates {
    (1,65.6)
    (2,66.4)
    (3,65.9)
    (4,66.0)
    (5, 66.3)
    (6, 65.8)
    (7,66.5)
    (8,66.2)
    (9,65.1)
};
\addplot[mark=diamond*,thick,blue] coordinates {
    (1,65.8)
    (2,66.9)
    (3,66.7)
    (4,66.0)
    (5, 65.5)
    (6, 66.4)
    (7,67.0)
    (8,65.9)
    (9,66.3)
};
\addplot[mark=diamond*,thick,cyan] coordinates {
    (1,68.7)
    (2,68.3)
    (3,69.0)
    (4,68.3)
    (5, 69.0)
    (6, 68.6)
    (7,68.6)
    (8,67.8)
    (9,68.2)
};

%\addlegendentry{$\beta=1$}
\addplot[mark=diamond*,thick,green] coordinates {
    (1,68.3)
    (2,68.4)
    (3,68.1)
    (4,68.6)
    (5, 68.8)
    (6, 69.2)
    (7,68.5)
    (8,69.4)
    (9,68.3)
};
\addplot[mark=diamond*,thick,red] coordinates {
    (1,68.9)
    (2,68.6)
    (3,68.8)
    (4,68.6)
    (5,68.4)
    (6,68.61)
    (7,68.8)
    (8,68.0)
    (9,68.7)
};
%\addlegendentry{$beta=100$}
\end{axis}
\end{tikzpicture}



\begin{tikzpicture}[every node/.style={scale=2}]
\begin{axis}[legend style={at={(.9,0.9),anchor=north east}},
             legend style={cells={anchor=west}, legend pos=outer north east,}, xtick={1,2,3,4,5,6,7,8,9}, xticklabels={0.5,1,2,5,7,10,15,20,30}, title={PubMed}, xlabel={$K/$\#nodes (\%)}, ytick={76,77,78,79,80}, ymin=76, ymax=80,
]

\addplot[mark=diamond*,thick,violet] coordinates {
    (1,77.2)
    (2,77.9)
    (3,77.8)
    (4,77.8)
    (5, 77.6)
    (6,76.8)
};
\addlegendentry{$\beta=1$}
\addplot[mark=diamond*,thick,blue] coordinates {
    (1,78.7)
    (2,78.2)
    (3,78.6)
    (4,78.6)
    (5, 78.6)
    (6,78.8) %%MISSING
};
\addlegendentry{$\beta=10$}
\addplot[mark=diamond*,thick,cyan] coordinates {
    (1,78.0)
    (2,78.4)
    (3,78.1)
    (4,78.4)
    (5, 78.4)
    (6,78.0)
};

\addlegendentry{$\beta=50$}
\addplot[mark=diamond*,thick,green] coordinates {
    (1,78.1)
    (2,78.6)
    (3,78.4)
    (4,78.3)
    (5, 77.9)
    (6,77.8)
};
\addlegendentry{$\beta=100$}
\addplot[mark=diamond*,thick,red] coordinates {
    (1,77.9)
    (2,78.1)
    (3,77.8)
    (4,78.2)
    (5, 78.1)
    (6,78.5)
};
\addlegendentry{$\beta=200$}
\end{axis}
\end{tikzpicture}

%int(0.005*n_nodes),int(0.01*n_nodes), int(0.02*n_nodes), int(0.05*n_nodes), int(0.07*n_nodes), int(0.1*n_nodes), int(0.15*n_nodes), int(0.2*n_nodes), int(0.3*n_nodes) 

% =================== K 13
% cora 0.8321999999999999 0.013197642887189252 cora 0.7913 0.016131749233524964
% cora 0.8309 0.012913816889930952 cora 0.7909 0.014858218825507552
% -------------------
% =================== time 8
% =================== K 27
% cora 0.8376 0.009640193635676282 cora 0.7963 0.01225697080576329
% cora 0.8371 0.008824838682818963 cora 0.7964 0.012712198865656575
% -------------------
% =================== time 7
% =================== K 54
% cora 0.8337 0.009661492868312051 cora 0.7871 0.015416081069959231
% cora 0.8345 0.00984603699182796 cora 0.7863 0.015783606122246652
% -------------------
% =================== time 8
% =================== K 135
% cora 0.8418 0.011013123484683585 cora 0.7958000000000001 0.01907179418233464
% cora 0.8429 0.010805862606320093 cora 0.7966 0.018056700818378877
% -------------------
% =================== time 8
% =================== K 189
% cora 0.831 0.009718253158075509 cora 0.7915000000000001 0.005797509043642034
% cora 0.8337 0.009989438867568541 cora 0.7904 0.006552353266829667
% -------------------
% =================== time 8
% =================== K 270
% cora 0.8356 0.015071680581658933 cora 0.7976000000000001 0.009845472732852065
% cora 0.8381 0.012431590583849034 cora 0.7975000000000001 0.008797095480264439
% -------------------
% =================== time 7
% =================== K 406
% cora 0.8371999999999999 0.00882924433660977 cora 0.7881 0.0168420769371107
% cora 0.8365 0.010013879257199878 cora 0.7883 0.014353087163084862
% -------------------
% =================== time 7
% =================== K 541
% cora 0.8319 0.014639748024546794 cora 0.7998000000000001 0.011593101396951537
% cora 0.8308 0.016551602809261563 cora 0.799 0.011547005383792502
% -------------------
% =================== time 7
% =================== K 812
% cora 0.8311 0.010857153299911446 cora 0.7886 0.017360235533476424
% cora 0.835 0.010154364141151886 cora 0.7878000000000001 0.01981469712668407
% -------------------
% =================== time 8
% /export/scratch/costas/anaconda3/envs/py37/lib/python3.7/site-packages/dgl/data/citation_graph.py:140: RuntimeWarning: divide by zero encountered in power
%   r_inv = np.power(rowsum, -1).flatten()
% Finished data loading and preprocessing.
%   NumNodes: 3327
%   NumEdges: 9228
%   NumFeats: 3703
%   NumClasses: 6
%   NumTrainingSamples: 120
%   NumValidationSamples: 500
%   NumTestSamples: 1000
% =================== K 16
% citeseer 0.6828000000000001 0.012821856339859652 citeseer 0.5865 0.010741922029548021
% citeseer 0.683 0.015070206073943061 citeseer 0.5883999999999999 0.011587349423689048
% -------------------
% =================== time 8
% =================== K 33
% citeseer 0.6841 0.010660935960578452 citeseer 0.5835 0.01670162999363967
% citeseer 0.6834 0.012694705808153045 citeseer 0.5836 0.015486194568783574
% -------------------
% =================== time 8
% =================== K 66
% citeseer 0.6804 0.013533497535949627 citeseer 0.5864 0.021975744204311566
% citeseer 0.6806 0.012615686884016854 citeseer 0.587 0.023701851779508242
% -------------------
% =================== time 8
% =================== K 166
% citeseer 0.6815 0.011664285471281774 citeseer 0.594 0.015705625319186314
% citeseer 0.6867 0.01019858377967796 citeseer 0.5928 0.017060676031935725
% -------------------
% =================== time 8
% =================== K 232
% citeseer 0.684 0.007086763875156399 citeseer 0.5826 0.020619300559319535
% citeseer 0.688 0.011095544651395459 citeseer 0.5824 0.020039960079800544
% -------------------
% =================== time 8
% =================== K 332
% citeseer 0.6924 0.009731963373909218 citeseer 0.5888 0.017611864687697803
% citeseer 0.6917 0.008420213774008319 citeseer 0.5894 0.01623576299408189
% -------------------
% =================== time 8
% =================== K 499
% citeseer 0.6852 0.017491585278514767 citeseer 0.5837 0.014275464576989734
% citeseer 0.6833 0.017531241953850373 citeseer 0.5834 0.014049120178067273
% -------------------
% =================== time 8
% =================== K 665
% citeseer 0.6944 0.009106774035482207 citeseer 0.5906 0.013825901618178682
% citeseer 0.6942999999999999 0.01170042734262298 citeseer 0.5906 0.013409780841692474
% -------------------
% =================== time 8
% =================== K 998
% citeseer 0.683 0.01319090595827289 citeseer 0.5809 0.018447824322185585
% citeseer 0.6817 0.013030306553910697 citeseer 0.5824 0.018482424083436668
% -------------------
% =================== time 8
% Finished data loading and preprocessing.
%   NumNodes: 19717
%   NumEdges: 88651
%   NumFeats: 500
%   NumClasses: 3
%   NumTrainingSamples: 60
%   NumValidationSamples: 500
%   NumTestSamples: 1000
% =================== K 98
% pubmed 0.7814 0.006785605679999725 pubmed 0.7454 0.018886797269815542
% pubmed 0.7809 0.006657493689236385 pubmed 0.7462 0.019937680685353346
% -------------------
% =================== time 9
% =================== K 197
% pubmed 0.7862 0.00981835016690687 pubmed 0.7452 0.01705416208567413
% pubmed 0.7868 0.01172651316935735 pubmed 0.7435 0.014562127439201867
% -------------------
% =================== time 10
% =================== K 394
% pubmed 0.784 0.00910433352249845 pubmed 0.7556 0.01108753053359194
% pubmed 0.785 0.009556847457887643 pubmed 0.7548 0.011448435118681806
% -------------------
% =================== time 10
% =================== K 985
% pubmed 0.7817000000000001 0.00812472221747373 pubmed 0.7514 0.0112368441595791
% pubmed 0.7829 0.009024041962077387 pubmed 0.7522 0.011545080722493417
% -------------------
% =================== time 12
% =================== K 1380
% pubmed 0.7771 0.006690789689316706 pubmed 0.7548 0.01902512958051945
% pubmed 0.779 0.0073484692283495405 pubmed 0.7548 0.0189373235231968
% -------------------
% =================== time 16
% =================== K 1971
% pubmed 0.7773 0.008819800955174047 pubmed 0.7479 0.010192044828089108
% pubmed 0.7786000000000001 0.010134649037392035 pubmed 0.7463 0.010078028907810637
% -------------------
% =================== time 19
